SafeCiM: Investigating Resilience of Hybrid Floating-Point Compute-in-Memory Deep Learning Accelerators

Deep Neural Networks (DNNs) continue to grow in complexity with Large Language Models (LLMs) incorporating vast numbers of parameters. Handling these parameters efficiently in traditional accelerators is limited by data-transmission bottlenecks, motivating Compute-in-Memory (CiM) architectures that integrate computation within or near memory to reduce data movement. Recent work has explored CiM designs using Floating-Point (FP) and Integer (INT) operations. FP computations typically deliver higher output quality due to their wider dynamic range and precision, benefiting precision-sensitive Generative AI applications. These include models such as LLMs, thus driving advancements in FP-CiM accelerators. However, the vulnerability of FP-CiM to hardware faults remains underexplored, posing a major reliability concern in mission-critical settings. To address this gap, we systematically analyze hardware fault effects in FP-CiM by introducing bit-flip faults at key computational stages, including digital multipliers, CiM memory cells, and digital adder trees. Experiments with Convolutional Neural Networks (CNNs) such as AlexNet and state-of-the-art LLMs including LLaMA-3.2-1B and Qwen-0.3B-Base reveal how faults at each stage affect inference accuracy. Notably, a single adder fault can reduce LLM accuracy to 0%. Based on these insights, we propose a fault-resilient design, SafeCiM, that mitigates fault impact far better than a naive FP-CiM with a pre-alignment stage. For example, with 4096 MAC units, SafeCiM reduces accuracy degradation by up to 49x for a single adder fault compared to the baseline FP-CiM architecture.

==> tables/Fault_inj.tex <==
\begin{table*}[]
\centering
    \caption{Fault Injection Experiments Summary}
    \label{tab:exp_summary}
\begin{tabular}{|lll|}
\hline
\multicolumn{1}{|c|}{\textbf{Fault Location}}    & \multicolumn{1}{c|}{\textbf{Fault Injection Experiment}}                                                                                           & \multicolumn{1}{c|}{\textbf{Experiment Findings}}                                                                                                                                                              \\ \hline
\multicolumn{3}{|l|}{\textbf{Input Pre-Alignment}}                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\multicolumn{1}{|l|}{Offsets}                    & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}4-bit offset values for input offset values\\ in the pre-alignment\end{tabular}}                    & \begin{tabular}[c]{@{}l@{}}Input offset bits are fault-sensitive, with MSB most \\ vulnerable. BERT shows resilience in LSBs due to \\ short sequences and GELU activation.\end{tabular}                       \\ \hline
\multicolumn{1}{|l|}{Exponents}                  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Maximum exponent value across all\\ groups at input pre-alignment\end{tabular}}                     & \begin{tabular}[c]{@{}l@{}}Input exponent faults cause severe degradation, \\ especially near MSB. BERT’s narrow exponent \\ range reduces LSB fault impact.\end{tabular}                                      \\ \hline
\multicolumn{3}{|l|}{\textbf{Weight Pre-Alignment}}                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{|l|}{Offsets}                    & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}4-bit offset values for weight offset values\\ in the pre-alignment\end{tabular}}                   & \begin{tabular}[c]{@{}l@{}}Weight offset faults are less impactful than input \\ offsets. Faults in MSB vary by model; LSB remains \\ low-risk across all models under test.\end{tabular}                      \\ \hline
\multicolumn{1}{|l|}{Exponents}                  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Maximum exponent value across all groups\\ at weight pre-alignment\end{tabular}}                    & \begin{tabular}[c]{@{}l@{}}Weight exponent faults are less severe than input \\ exponents. Sensitivity varies by bit and model; no \\ consistent MSB-to-LSB trend.\end{tabular}                                \\ \hline
\multicolumn{3}{|l|}{\textbf{CiM Crossbar}}                                                                                                                                                                                                                                                                                                                                                                            \\ \hline
\multicolumn{1}{|l|}{CiM Memory Cells}           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Bits 13 (MSB), 11, 8, 6 of the pre-aligned\\ weight mantissas programmed to CiM\end{tabular}}       & \begin{tabular}[c]{@{}l@{}}MSB faults in weight mantissas cause major \\ accuracy loss. LSB faults are negligible, emphasizing \\ protection of high-order bits.\end{tabular}                                  \\ \hline
\multicolumn{1}{|l|}{CiM Multipliers}            & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Bits 26 (MSB), 25, 21, 11, 6 of the\\ elementwise products from the\\ CiM multipliers\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Multiplier MSB faults degrade accuracy faster than \\ memory faults.\end{tabular}                                                                                                   \\ \hline
\multicolumn{3}{|l|}{\textbf{CiM Adder Tree}}                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{1}{|l|}{Adder}                      & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Bits MSB, MSB-1, 26, 21, 11, 6 of a\\ randomly selected adder at a\\ given level\end{tabular}}      & \begin{tabular}[c]{@{}l@{}}Adder faults compound across summation levels. \\ A single MSB fault can collapse accuracy; bit 26 \\ sensitivity changes post-alignment.\end{tabular}                              \\ \hline
\multicolumn{1}{|l|}{Global Alignment Offsets}   & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}4-bit offset values for mantissa sums\\ in global alignment\end{tabular}}                           & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Global alignment is highly vulnerable. Bits 3 and 4 \\ of the global exponents are most impactful due to \\ exponent rollover near the 235–250 range.\end{tabular}} \\ \cline{1-2}
\multicolumn{1}{|l|}{Global Alignment Exponents} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Sum of maximum exponents of inputs\\ and weights from pre-alignment\end{tabular}}                   &                                                                                                                                                                                                                \\ \hline
\multicolumn{3}{|l|}{\textbf{Normalization}}                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
\multicolumn{1}{|l|}{Sign and Exponent}          & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Bits MSB till bit 8 in the normalized\\ FP partial sum\end{tabular}}                                & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Normalization is the most fault-sensitive stage. \\ Exponent faults lead to NaNs;  BERT shows \\ high mantissa sensitivity.\end{tabular}}                           \\ \cline{1-2}
\multicolumn{1}{|l|}{Mantissa}                   & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Bits 7 till LSB (bit 1) in the normalized\\ FP partial sum\end{tabular}}                            &                                                                                                                                                                                                                \\ \hline
\end{tabular}
\end{table*}

==> tables/Tab_fault_injection.tex <==
\begin{table*}[]
\caption{Summary of fault injection operations in FaultCiM for FP CiM datapath.}
\begin{tabular}{|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{FP CiM Compute Stage}}                                     & \multicolumn{1}{c|}{\textbf{Fault Type at Target Bits}}                                                                                                                                                                                                                                                                                                                                                   & \multicolumn{1}{c|}{\textbf{Effect Summary}}                                                                           \\ \hline
\begin{tabular}[c]{@{}l@{}}Pre-Alignment Exponents \\ (Inputs and Weights)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Single bit-flip in unsigned exponent bits \\ (refer Figure~\ref{fig:fault_modeling} \tikz[baseline=-0.5ex] \node[circle, fill=black, text=white, inner sep=0.5mm]{1}; and \tikz[baseline=-0.5ex] \node[circle, fill=black, text=white, inner sep=0.5mm]{2};)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Misaligned mantissas due to incorrect \\ exponent selection\end{tabular}                    \\ \hline
\begin{tabular}[c]{@{}l@{}}Pre-Alignment Offsets \\ (Inputs and Weights)\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Single bit-flip in unsigned offset bits \\ (refer Figure~\ref{fig:fault_modeling} \tikz[baseline=-0.5ex] \node[circle, fill=black, text=white, inner sep=0.5mm]{1}; and \tikz[baseline=-0.5ex] \node[circle, fill=black, text=white, inner sep=0.5mm]{2};)\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Incorrect mantissa shift amount before \\ storage in CiM memory\end{tabular}                \\ \hline
CiM Memory                                                                              & \begin{tabular}[c]{@{}l@{}}2's complement programmed \\ mantissas with bit-flip fault (refer Figure~\ref{fig:fault_modeling} \tikz[baseline=-0.5ex] \node[circle, fill=black, text=white, inner sep=0.5mm]{3}; )\end{tabular}                                                                                                                 & Corrupts weights before multiplication                                                                                 \\ \hline
CiM Multipliers                                                                         & \begin{tabular}[c]{@{}l@{}}Bit-flip fault in elementwise \\ multiplier outputs (refer Figure~\ref{fig:fault_modeling} \tikz[baseline=-0.5ex] \node[circle, fill=black, text=white, inner sep=0.5mm]{3};)\end{tabular}                                                                                                                         & Corrupts the multiplication output                                                                                     \\ \hline
CiM Adder                                                                               & \begin{tabular}[c]{@{}l@{}}Output of an adder within the \\ adder tree injected with bit-flip fault (refer Figure~\ref{fig:fault_modeling} \tikz[baseline=-0.5ex] \node[circle, fill=black, text=white, inner sep=0.5mm]{4};)\end{tabular}                                                                                                    & \begin{tabular}[c]{@{}l@{}}Error introduced and propagated during \\ accumulation of elementwise products\end{tabular} \\ \hline
Global Alignment Offsets                                                                & \begin{tabular}[c]{@{}l@{}}Bit-flip fault in the unsigned \\ offsets at global alignment (refer Figure~\ref{fig:fault_modeling} \tikz[baseline=-0.5ex] \node[circle, fill=black, text=white, inner sep=0.5mm]{5};)\end{tabular}                                                                                                               & Misalignment across adder outputs                                                                                      \\ \hline
Global Alignment Exponents                                                              & \begin{tabular}[c]{@{}l@{}}Bit-flip fault in the exponent sums \\ (refer Figure~\ref{fig:fault_modeling} \tikz[baseline=-0.5ex] \node[circle, fill=black, text=white, inner sep=0.5mm]{5};)\end{tabular}                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Incorrect global exponent affects all \\ alignments\end{tabular}                                                                       \\ \hline
Normalization                                                                           & \begin{tabular}[c]{@{}l@{}}Bit-flip fault at any of the sign, \\ exponent or mantissa bits (refer Figure~\ref{fig:fault_modeling} \tikz[baseline=-0.5ex] \node[circle, fill=black, text=white, inner sep=0.5mm]{6};)\end{tabular}                                                                                                             & \begin{tabular}[c]{@{}l@{}}Final FP output corruption or Not-a-Number \\ (NaN)\end{tabular}                                                                        \\ \hline
\end{tabular}
\label{tab:fault_summary}
\end{table*}
